MSG-BART: Multi-granularity Scene Graph-Enhanced Encoder-Decoder Language Model for Video-grounded Dialogue Generation

Generating dialogue grounded in videos requires a high level of understanding and reasoning about the visual scenes in the videos. However, existing large visual-language models are not effective due to their latent features and decoder-only structure, especially with respect to spatio-temporal relationship reasoning. In this paper, we propose a novel approach named MSG-BART, which enhances the integration of video information by incorporating a multi-granularity spatio-temporal scene graph into an encoder-decoder pre-trained language model. Specifically, we integrate the global and local scene graph into the encoder and decoder, respectively, to improve both overall perception and target reasoning capability. To further improve the information selection capability, we propose a multi-pointer network to facilitate selection between text and video. Extensive experiments are conducted on three video-grounded dialogue benchmarks, which show the significant superiority of the proposed MSG-BART compared to a range of state-of-the-art approaches.

==> 02Related_Works.tex <==
\section{Related Works}
In this section, we will review prior works that are relevant to our proposed method including the Video-grounded Dialogues, scene graph, and pointer network.

\subsection{Video-grounded Dialogues}

The Video-grounded Dialogues (VGD) task is to answer questions based on the content of the video and the dialogue history and requires perceiving the space-time relationships of dynamic scenes. Compared to other visual dialogue tasks, VGD has a greater diversity in responses \citep{avsd}, which requires strong spatio-temporal reasoning and information integration ability between video and dialogue. That is why most methods focus on the overall perception of videos (i.e., cross attention \citep{av-trans}, concatenation \citep{med-cat}). And various methods have been proposed to enhance the capability of local perception, including question-aware attention \citep{hori2019end}, hierarchical attention \citep{le2019multimodal}, and memory network \citep{DialogMCF}.
Despite recent progress, most methods ignore the importance of the interaction between the global feature and local feature as well as the encoder and decoder. In this paper, we propose to enhance pre-trained language models consisting of the ED structure with multi-granularity video feature injection during the encoding stage and the decoding stage, to establish the overall perception of videos and local perception of the question-relevant portion in videos.


\subsection{Scene Graph}
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{image/scene-graph.pdf}
\caption{The demonstration of the scene graph. Entities are identified from pictures or video clips, and entities are divided into spatial, contact, and attention relationships with each other.}
\label{fig:sce}
\end{figure}
The scene graph is used to represent the image by diagram structure, which is shown in Figure~\ref{fig:sce}.
% Visual Genome \citep{krishna2017visual} is widely used due to the large size of the data and the rich semantic information it contains. To introduce scene graphs to video tasks, \cite{ji2020action} extend the scene graph to the dynamic scene graph. 
It is widely used in multimodal dialogue because it can effectively structure visual information. 
% \cite{cherian20222} represent the  video by a (2.5+1)D spatio-temporal scene graph for better reasoning of the video information. 
\cite{geng2021dynamic}, \cite{jiang2020dualvd}, and \cite{guo2020iterative} make multimodal reasoning via graph attention networks using symbolic or latent overall scene graph representations. \cite{wang2020ord} use local graph convolutional networks to obtain a better global graph representation and inject the global representation into the encoder, which gains a lot in visual dialogue. However, existing works ignore the interaction between the global feature and the local feature. In this paper, we propose the multi-granularity spatio-temporal scene graph which captures both node and triplet-level information to better capture the knowledge of the video.

\subsection{Pointer Network}
The pointer network \citep{pointer} is proposed to solve the problem that the target dictionary varies depending on the input sequences. Based on this model, the Pointer-Generator Network is proposed for text summarization by combining different source information, which is extended for external information selection and fusion in \citep{liu2022improving}.  For text generation tasks, \cite{chen2021jointly}, \cite{guo2022lexicon}, and \cite{le2020multimodal} take advantage of the pointer to select relevant information. For VGD, it is important to select and incorporate the information adaptively according to different questions, which is often neglected in the existing works. In this paper, we propose a novel multi-pointer that is based pointer-generator network, for more powerful information selection. 



==> 06Limitation.tex <==
\section*{Limitations}
 Although our model is significantly more effective than the state-of-the-art models, there are still some limitations: 1) It does not make good use of audio information and does not effectively eliminate audio noise, we will focus on other information carriers similar to scene graphs to represent the audio information. 2) Despite the introduction of scene graphs, the generation of scene graphs is fixed and a rather general instead of question-oriented method is used, we will improve the generation of the scene graph which can be guided by questions in the future. 3)  We conduct the experiment on large language models which is shown in Appendix~\ref{sec:appendix_llm}. Due to the computational resources, we cannot compare the large language model (LLM) with single granularity video features and LLM with our method in a fair situation. In the future, we will do more experiments with a larger language model than BART-base (i.e. T5-large (738M), T5-xl (3B)) to further validate the superiority of our proposed approach.

 % We use a cross-modal spatio-temporal scene graph, capturing the information of the video into a  symbolic scene graph, and we will consider combining both symbolic and latent graph representation for dialogue generation in the future.
 % With consideration of the computing cost and application situation, we use the greedy search as the sampling strategy in AVSD-LLaMA-7B. It cannot truly demonstrate that the MSG-BART  outperforms AVSD-LLaMA-7B. Considering the model size difference of 50 times, it can indicate the superiority of our model in a certain sense. In the future, we will do more experiments to prove it.
